Do LLMs Provide Links to Code Similar to what they Generate? A Study with Gemini and Bing CoPilot

Large Language Models (LLMs) are currently used for various software development tasks, including generating code snippets to solve specific problems. Unlike reuse from the Web, LLMs are limited in providing provenance information about the generated code, which may have important trustworthiness and legal consequences. While LLM-based assistants may provide external links that are "related" to the generated code, we do not know how relevant such links are. This paper presents the findings of an empirical study assessing the extent to which 243 and 194 code snippets, across six programming languages, generated by Bing CoPilot and Google Gemini, likely originate from the links provided by these two LLM-based assistants. The study leverages automated code similarity assessments with thorough manual analysis. The study's findings indicate that the LLM-based assistants provide a mix of relevant and irrelevant links having a different nature. Specifically, although 66% of the links from Bing CoPilot and 28% from Google Gemini are relevant, LLMs-based assistants still suffer from serious "provenance debt".

==> indistrialApp.tex <==
\begin{figure}
\includegraphics[width=\linewidth]{troubleshooterRAG/img/production.pdf}
    \caption{Integrating the troubleshooter in the CI/CD pipeline.}
    \label{fig:production}
    %\vspace{-2mm}
\end{figure}

%\MAX{expand by explaining: new models being experimented, novel results, if possible a screenshot of the application working. Ideally, also updated results with practitioners, and a summary of the results of the new questionnaire.}

After receiving positive feedback from the evaluators, the proposed troubleshooter has been made available to developers.

More specifically, the troubleshooter has been integrated into a CI/CD pipeline,
%\footnote{Specific technology omitted based on corporate regulations.}, 
as depicted in \figref{fig:production}. 
Whenever a build deploying a microservice fails, the troubleshooter is automatically invoked by reading the build failure from the CI/CD infrastructure. Then, the generated solution proposal is automatically appended---as a comment---to the build log so developers can browse it by accessing the log through the web-based pipeline dashboard.

The production troubleshooter is using the same knowledge base used in our evaluation, yet it could be extended with data from previously applied solutions. The main reason why this was not done is because the pipeline works on customer's build failures, which we have preferred not to seed into the knowledge base. However, instead of considering only the top-1 results, it dynamically considers up to three topmost relevant results, provided that they fit the context length for LLama-2.

Further, we have introduced a different LLM, Claude 2.1 \cite{claude}, which has proven superior to Llama2. To make this transition, we conducted several internal surveys to evaluate whether Claude 2.1 offered improvements. More specifically, we compared Llama2-13b, Llama2-70b, and Claude 2.1 through surveys with our experts, and Claude 2.1 emerged as the best.

To ensure a high degree of customer data security and service quality, we perform model inference using the new AWS Bedrock service. This service ensures reduced latency times, continuous support from Amazon, and security for the data sent to the model.

The continued use of this approach and the various analyses conducted with both Llama2 and Claude 2.1, have highlighted how the RAG (Retrieval Augmented Generation) approach, leveraging information from Stack Exchange, combined with a custom template solution, has substantially improved the troubleshooter's responses both qualitatively and descriptively, as well as the proposed code to solve issues.

%In terms of LLM, we opted for Llama-2 given its superior performance with respect to other models we considered. Also, we have equipped the production tool with a larger (13b) version of the LLama-2 model.

==> macro.tex <==
\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter


\newcommand{\COMMENT}[1]{}
\newcommand{\ndef}{\stackrel{\rm def}{=}}
\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}


\newcommand\NEW[1]{\nb{NEW}{#1}}
\newcommand{\numLib}{12\xspace}


\usepackage{xspace}


\sloppy

\newcommand{\rev}[1]{\textcolor{black}{#1}}
\newcommand{\tool}[1]{\textsc{#1}\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\etc}{etc.\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\secref}[1]{Section~\ref{#1}\xspace}
\newcommand{\chapref}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\appref}[1]{Appendix~\ref{#1}\xspace}
\newcommand{\figref}[1]{Figure~\ref{#1}\xspace}
\newcommand{\listref}[1]{Listing~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}
\newcommand{\hf}{HF\xspace}
\newtcolorbox{resultbox}{colback=gray, arc=0.5mm, top=1mm, bottom=1mm, left=1mm, right=1mm}
\newboolean{showcomments}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{javapurple}{rgb}{1,0.5,0.31} % keywords
\definecolor{javablue}{rgb}{0.25,0.35,0.75}
\definecolor{backbefore}{rgb}{0.94,0.63,0.63}
\definecolor{backafter}{rgb}{0.6,1,0.6}





\definecolor{gray}{rgb}{0.83,0.83,0.83}
\definecolor{green}{rgb}{0.56,0.93,0.56}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\newcommand*\circleds[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=0pt] (char) {#1};}}

\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
{\newcommand{\nb}[2]{
		\fbox{\bfseries\sffamily\scriptsize#1}
		{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
	}
}
{\newcommand{\nb}[2]{}
}

%comments
\newcommand\MAX[1]{\textcolor{blue}{\nb{MAX}{#1}}}
\newcommand\DANIELE[1]{\textcolor{green}{\nb{DANIELE}{#1}}}
\newcommand\PIETRO[1]{\textcolor{red}{\nb{PIETRO}{#1}}}
\newcommand\TODO[1]{\textcolor{orange}{\nb{TODO}{#1}}}
\newcommand\FIORELLA[1]{\textcolor{brown}{\nb{FIORELLA}{#1}}}
\newcommand\GIUSEPPE[1]{\textcolor{violet}{\nb{GIUSEPPE}{#1}}}
\newcommand\revised[1]{\textcolor{black}{#1}}
\newcommand{\bcp}{Bing CoPilot\xspace}
\newcommand{\gem}{Gemini\xspace}

% Values
\newcommand{\lang}{six\xspace}

\newcommand{\queries}{278\xspace}
\newcommand{\cNTqueries}{175\xspace}
\newcommand{\gNTqueries}{173\xspace}

\newcommand{\cSnip}{243\xspace}
\newcommand{\gSnip}{194\xspace}

%the total amount of sources provided by the LLM
%including the sources related to all trivial generated snippet
\newcommand{\cWTSources}{1,516\xspace}
\newcommand{\gWTSources}{704\xspace}
\newcommand{\WTSources}{2,220\xspace}

%the number of sources related to queries with at least one NON-Trivial snippet
\newcommand{\cSources}{1,006\xspace}
\newcommand{\gSources}{514\xspace}
\newcommand{\Sources}{1,520\xspace}

% RQ
\newcommand{\rqone}{To what extent are LLM-based assistants able to provide links to external sources for code generation tasks?}
\newcommand{\rqtwo}{To what extent are the automatically generated code snippets ``similar'' to code snippets extracted from the LLM-provided links?}
%sources?}
